Enhancing Dexterity in Robotic Manipulation via Hierarchical Contact Exploration

Planning robot dexterity is challenging due to the non-smoothness introduced by contacts, intricate fine motions, and ever-changing scenarios. We present a hierarchical planning framework for dexterous robotic manipulation (HiDex). This framework explores in-hand and extrinsic dexterity by leveraging contacts. It generates rigid-body motions and complex contact sequences. Our framework is based on Monte-Carlo Tree Search and has three levels: 1) planning object motions and environment contact modes; 2) planning robot contacts; 3) path evaluation and control optimization. This framework offers two main advantages. First, it allows efficient global reasoning over high-dimensional complex space created by contacts. It solves a diverse set of manipulation tasks that require dexterity, both intrinsic (using the fingers) and extrinsic (also using the environment), mostly in seconds. Second, our framework allows the incorporation of expert knowledge and customizable setups in task mechanics and models. It requires minor modifications to accommodate different scenarios and robots. Hence, it provides a flexible and generalizable solution for various manipulation tasks. As examples, we analyze the results on 7 hand configurations and 15 scenarios. We demonstrate 8 tasks on two robot platforms.

==> sections/2_related.tex <==
\section{Related Work}

\subsection{Dexterous Manipulation Planning}
Most works in manipulation focus on individual skills, like pushing \cite{mason1986mechanics}\cite{lynch1996stable}, pivoting \cite{aiyama1993pivot,holladay2015general,hou2018fast,cheng2019suctioncups}, tumbling \cite{maeda2004motion}, grasping \cite{eppner2015exploitation}\cite{eppner2015planning}, on-table reorientation \cite{hou2018fast}, and predefined dynamic skills \cite{woodruff2017planning}. 
While the mechanics and planning of specific motion types are studied in depth, generating dexterous manipulation planning is still under-explored. 

What are the essential challenges about dexterous manipulation planning? 
The presence of potential contact changes introduce discontinuity and changes in system dynamics (non-differentiable). This leaves us a high dimensional, non-convex, discrete and continuous space to plan through. 

Contact-implicit trajectory optimization (CITO) \cite{posa2014direct} directly solves nonlinear programming (NLP) problems in the complex hybrid space. Most methods simplify the problems to make them tractable. Simplifications include simple primitive shape representation\cite{mordatch2012contact,mordatch2012discovery}, reducing to 2D, and small number of contact transitions \cite{Sleiman2019CIO,doshi2020icra,aceituno-cabezas2020rss}. Moreover, CITO can be slow and intractable without good initialization. 

It is worth to explore the space through global search. To capture the discreteness of manipulation systems, previous research searches through predefined manipulation modes and solve for each mode sequence the whole trajectory using an NLP \cite{toussaint2018differentiable}. 
For dexterous manipulation, manually defining modes could be engineering heavy or even intractable, as suggested by observations in dexterous grasping \cite{nakamura2017complexities}. 
Alternatively, expert knowledge in contacts, like contact formations \cite{xiao2001automatic}, contact states \cite{ji2001planning} and contact modes \cite{Mason, huang2020efficient} are exploited to efficiently generate rigid body motions between two bodies~\cite{tang2008automatic}, within a robot hand~\cite{trinkle1991dexterous, yashima2003randomized}, dexterous pregrasps \cite{chen2023pregrasp}, under environment contacts \cite{cheng2020contact, cheng2022contact3D, liang2022learning}, and with local trajectory optimization combined with high-level planning \cite{pang2022global, chen2021trajectotree}. Contact modes can help guide automatically generation of motion primitives that are differentiable in dynamics \cite{huang2023autogenerated}. 

Built on the idea of exploiting contacts, our work pushes forward towards a more general framework in 3D dexterous manipulation. 
We exploit hierarchies inspired by previous hierarchical frameworks for 2D manipulation \cite{lee2015hierarchical, aceituno2022hierarchical}. 
While we share a similar idea of decomposing the search in object motions and robot contacts, we design different pipelines, efficient exploration of contacts, and new representations to make it feasible for complex 3D scenarios. 

Reinforcement learning (RL) is efficient in discovering manipulation skills from direct interactions with the environment, like in-hand manipulation \cite{andrychowicz2020learning}, dexterous grasping \cite{zhou2022learning}, and multi-step object reorientation \cite{zhou2023learning}. RL faces the same challenges from high-dimensional complex spaces, leading to sample efficiency problems. 
RL also requires significant training for new tasks, while our planners can be directly used for a new object or environment. 
% For future research, as \cite{grill2020monte} shows that MCTS is an approximation of regularized policy optimization algorithms, we hope to combine our framework with RL to leverage the strength of both.
For future research, we hope to combine our framework with RL to leverage the strength of both.

\subsection{Monte-Carlo Tree Search}
MCTS is a heuristic search algorithm that uses random sampling for efficient exploration. The AlphaGo family of algorithms \cite{silver2016alphago, silver2017mastering} combines MCTS with deep neural networks, achieving a superhuman level of play in board games like Go. MCTS has also shown it effectiveness in robotic applications such as robot task planning \cite{kartal2016monte}, task and motion planning \cite{ren2021extended}, and object rearrangement planning \cite{huang2019large,labbe2020monte}. 
MCTS has also shown potentials to plan in the large combinatoric space for contacts. Previous works include gait planning for legged robots \cite{amatucci2022mctslegged} and robot contact sequence planning given user-designed object trajectories\cite{zhu2022efficient}. 
% Both of them outperform Mixed-integer programming and 
% They have shown the potential of using MCTS for the large combinatoric space for contacts. 
Based on these works, our work takes one step further in planning not only robot contacts, but also object interactions with environment contacts (exploiting extrinsic dexterity\cite{dafle2014extrinsic}). %, which is considered hard to plan through \cite{posa2014direct}. 

The incorporation of MCTS also offers several current and future benefits, including efficient search through vast complex space, potentials for continuous improvement through deep learning and self-exploration \cite{silver2017mastering}, and parallelizability to accelerate the search \cite{chaslot2008parallel}.
